Log-Likelihood Ratio Minimizing Flows: Towards Robust and Quantifiable Neural Distribution Alignment

Distribution alignment has many applications in deep learning, including domain adaptation and unsupervised image-to-image translation. Most prior work on unsupervised distribution alignment relies either on minimizing simple non-parametric statistical distances such as maximum mean discrepancy or on adversarial alignment. However, the former fails to capture the structure of complex real-world distributions, while the latter is difficult to train and does not provide any universal convergence guarantees or automatic quantitative validation procedures. In this paper, we propose a new distribution alignment method based on a log-likelihood ratio statistic and normalizing flows. We show that, under certain assumptions, this combination yields a deep neural likelihood-based minimization objective that attains a known lower bound upon convergence. We experimentally verify that minimizing the resulting objective results in domain alignment that preserves the local structure of input domains.

==> figs/fig1.tex <==

\begin{figure}[t]
\begin{center}
\subfloat{\includegraphics[trim=20 190 300 0,width=0.5\textwidth]{imgs/figs/fig1_arrow.pdf}}
\subfloat{\includegraphics[trim=0 210 320 0,width=0.5\textwidth]{imgs/figs/fig_1_1.pdf}}
\caption{In the space of probability distributions over $\mathcal X \subset \mathbb R^n$, empirical distributions of datasets $A$ and $B$ can be thought of as points, and the parametric density family $M(\theta)$ as a surface. We want to find a transformation $T(x)$ that makes $A' \triangleq T(A)$ and $B$ ``equivalent'' with respect to $M$. More specifically, we want the optimal density estimator $\theta_{AT}$ for the transformed dataset $A'$ to be optimal for $B$ as well, like it is for $A^*$ and $B$. The majority of prior work on aligning datasets with respect to a given family of discriminating functions either severely restricts that family, or relies on adversarial training. In this paper, we show that if $T(x)$ is a family of normalizing flows, then, for an arbitrary family of densities $M(\theta)$, the optimal $T^*$ that makes $T^*(A)$ and $B$ share a projection onto $M$ can be found by solving a simple non-adversarial minimization problem (Eq~\ref{eq:lrmf_loss}).
% \vspace*{-20px}
}
\label{fig:prob_space}
\vspace{-15px} 
% In the space of all probability distributions over $\mathcal X$, two datasets $A$ and $B$ can be thought of as points, and the parametric family of densities $\mathcal M(\theta)$ as a curve. Some points (probability distributions) in this space might have multiple optimal KL projections onto $\mathcal M$. We can think of two points (distributions) as equivalent ``with respect to $\mathcal M$'' if they share at least one such projection, e.g. distributions with equal means and variances are equivalent wrt normal distribution family. We would like to find a transformation $T(x)$ that makes $A' = T(A)$ and $B$ equivalent wrt $\mathcal M$. We notice that the combined distance from $A'$ and $B$ to their respective projections $\mathcal M(\theta_{AT})$ and $\mathcal M(\theta_B)$ \textbf{(2+5)} is always less then or equals the combined distance to a single ``shared'' approximation $\mathcal M(\theta_S)$ \textbf{(3+4)}. Datasets $B$ and $C$ are more similar wrt $\mathcal M$, and the difference between the combined distance to the optimal ``shared'' \textbf{(6+7)} and the ``private'' approximations \textbf{(5+8)} is smaller. This difference vanishes if densities are equivalent wrt $\mathcal M$. In general, the $T(x)$ that makes it vanish can be found only by solving a min-max optimization problem, but in this paper we show that if $T(x; \phi)$ is a family of normalizing flows, the optimal $\phi^*$ can be found by minimizating a single simple objective.
% We would like to find a transformation $T(x)$ such that the transformed dataset $A' = T(A)$ is in some sense equivalent to the dataset $B$. In this paper we introduce the manifold of density models $\mathcal M(\theta)$ and define the log-likelihood ratio distance $d_{\Lambda}$ between $A'$ and $B$ as the minimal combined distance (KL-divergence) from $A'$ and $B$ to a shared model $\theta_S$ across $M$, minus the combined minimal distances from $A'$ and $B$ to their respective optimal approximations on $M$, namely $\theta_{AT}$ and $\theta_{B}$ , i.e. $d_{\Lambda}(A', B) =\ $\textbf{(3)+(4)-(2)-(5)}. This quantity is always non-negative and equals zero only if there exists a single shared model that optimally approximates both datasets, i.e. if a single shared approximation is as good as two private approximations. For example, $d_{\Lambda}(C, B) =\ $ \textbf{(7)+(6)-(8)-(5)} is much smaller because the shared model $\theta_{BC}$ approximates both $B$ and $C$ almost as good as their ``private'' models $\theta_B$ and $\theta_C$. In general, the problem of finding $T$ that minimizes $d_{\Lambda}$ is still adversarial in nature, but in this paper we show that if $T(x; \phi)$ is a parametric normalizing flow, then the optimal $\phi^*$ can be found using plain minimization.
% }
\end{center}
\end{figure}

==> figs/fig1_v2.tex <==
\begin{figure*}
\vspace{-40px}
\begin{center}
\subfloat[Log-Likelihood Ratio Distance]{\includegraphics[trim=10 230 390 0,width=0.45\textwidth,valign=m]{imgs/figs/fig_1_1_v2.pdf}}\quad
\subfloat[Composition of flows and the local structure]{\includegraphics[trim=8 265 360 0,width=0.50\textwidth,valign=m]{imgs/figs/fig3_narrow.pdf}
\vphantom{\includegraphics[trim=10 230 390 0,width=0.45\textwidth,frame,valign=m]{imgs/figs/fig_1_1_v2.pdf}}
}
\caption{\textbf{(a)} The log-likelihood ratio distance between the fixed dataset $B$ and the transformed dataset $A'$ equals the difference between the average log-likelihoods of $A'$ and $B$ according to their ``private'' models (height of green and orange circles) and their log-likelihoods given the shared model (height of purple circles). The increase in average ``private'' log-likelihood of $A'$ relative to $A$ can estimated in closed form if $T$ is a normalizing flow. \textbf{(b)} If we train two normalizing flows ($G$ and $F$) on vertices of two meshes ($A$ and $B$ respectively), the marginal distribution of vertices in $F(G^{-1}(A))$ matches $B$, but the local structure of the manifold is distorted. Training a separate flow $T$ using the likelihood objective preserves the local structure. \vspace{-20px}}
\label{fig:fig1_mesh}
\end{center}
\end{figure*}


% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{center}
% \includegraphics[trim=0 270 360 10,width=0.45\textwidth]{imgs/figs/fig3_narrow.pdf}
% \caption{If we train two normalizing flows: $G$ on vertices of the mesh $A$ and $F$ on vertices of $B$, the marginal vertex distribution of $F(G^{-1}(A))$ matches $B$, but the local structure of the original manifold is distorted. On the other hand, training a separate flow $T$ to match $T(A)$ with $B$ using the likelihood objective preserves the local structure.
% % \vspace{-20px}
% }
% \label{fig:mesh_f_g_inv}
% \end{center}
% \end{wrapfigure}

==> figs/fig3_narrow.tex <==
\begin{figure*}
\vspace{-40px}
\begin{center}
\includegraphics[trim=0 270 360 10,width=0.45\textwidth]{imgs/figs/fig3_narrow.pdf}
\caption{If we train two normalizing flows: $G$ on vertices of the mesh $A$ and $F$ on vertices of $B$, the marginal vertex distribution of $F(G^{-1}(A))$ matches $B$, but the local structure of the original manifold is distorted. On the other hand, training a separate flow $T$ to match $T(A)$ with $B$ using the likelihood objective preserves the local structure. \vspace{-20px}}
\label{fig:mesh_f_g_inv}
\end{center}
\end{figure*}


% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{center}
% \includegraphics[trim=0 270 360 10,width=0.45\textwidth]{imgs/figs/fig3_narrow.pdf}
% \caption{If we train two normalizing flows: $G$ on vertices of the mesh $A$ and $F$ on vertices of $B$, the marginal vertex distribution of $F(G^{-1}(A))$ matches $B$, but the local structure of the original manifold is distorted. On the other hand, training a separate flow $T$ to match $T(A)$ with $B$ using the likelihood objective preserves the local structure.
% % \vspace{-20px}
% }
% \label{fig:mesh_f_g_inv}
% \end{center}
% \end{wrapfigure}

==> figs/fig_dyn_gauss_lrmf.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[trim=0 150 420 0,width=0.35\textwidth]{imgs/figs/fig2.pdf}
\caption{Optimizing the log-likelihood ratio distance (Eq 1) between the transformed dataset $A'$ and the target dataset $B$ with respect to the transformation parameter $\phi$ results in the dataset being pulled towards the shared model $\theta_S$ (green) and away from the best approximating model $\theta_{AT}$ (blue), resulting in the total combined gradient (black) that points towards the target dataset $B$. \vspace{-20px}}
\end{center}
\label{fig:llrd_adv_min}
\end{figure}

==> old/3_method_new_old.tex <==
\section{Method}

In this section we introduce the log-likelihood ratio pseudo-distance $d_\Lambda(\mu, \nu, T)$ between a fixed probability distribution $\mu$ and a transformed (push-forward) distribution $T(\nu)$ with respect to the specific family of densities $\mathcal F$. Intuitively, it equals zero if and only if the best approximation for $\mu$ from $\mathcal F$ is also optimal for $T(\nu)$ and vice versa. Or equivalently, if the entropy of the best approximation of $\mu$ does not change if we start mixing-in some points from $T(\nu)$. 

For example, if $\mathcal F$ is the Gaussian family of distributions, and $\mu$ is the Laplace density with zero mean and unit variance, and $\nu$ is the student's t-distribution with mean $A$ and unit variance, and $T(x; s) = x-s$ is the shift transformation, then the log-likelihood ratio pseudo-distance is going to equal zero only for $T(x; A)$ because for any other choice of the shift parameter $s$ the entropy of the best fit Gaussian to the mixture of $\mu$ and $T(\nu; s)$ is going to exceed the entropy of the best fit Gaussian for $\mu$ (a unit Gaussian). In this sense, all zero mean unit variance distributions are equivalent wrt log-likelihood ratio pseudo-distance with respect to the Gaussian family of distributions. In this paper we extend this concept far beyond the affine transformations and Gaussian densities.

Moreover, we show that if the transformation $T(x; \theta)$ is a normalizing flow parameterized with $\theta$ and rich enough to represent the transformation ``from $\nu$ to $\mu$'', then the otherwise adversarial log-likelihood ratio distance minimization turns into the plain minimization problem with known stopping criteria that can be optimized using conventional gradient decent.

\begin{notation} Consider a family of parametric densities $\mathcal F$ over the domain $\mathcal X$ with the log-likelihood $l_F(x; \theta)$ and a parametric normalizing flow $${T(x; \theta): \mathcal X \times \Theta \to \mathcal X}$$ with the associated log-likelihood function $l_T(x; \theta)$ and the latent prior log-likelihood $l_Z(x)$.
% $$ l_T(x; \theta) = \log \det | \nabla_{x} T(x; \theta) | + l_Z(T(x; \theta)).$$
\end{notation}

\begin{definition}
The pushforward measure later referred as $T(\mu; \theta)$ for short is defined as
$$ \big[T(\mu; \theta)\big](X) = \mu(T^{-1}(X; \theta_T))$$
\end{definition}

\begin{definition}
The combined model for a pair of random variables $A, B$ independently taking values $a, b$ from $\mathcal X$ is defined by the log-likelihood:
\begin{gather}
\begin{aligned}
\begin{split}
\label{eq:m_def}
  & g_F(a, b; \theta_T, \theta_A, \theta_{BT}) = \\
  & = \log \Pr(A=a, B=b \ | \ \theta_T, \theta_A, \theta_{BT}) \\
  & =  \log \Pr(A=a \ | \ \theta_A) + \log \Pr(B=T(b; \theta_T) \ | \ \theta_{BT}) \\
  & = l_F(a; \theta_A) + l_F(T(b; \theta_T); \theta_{BT})
\end{split}
\end{aligned}
\end{gather}
% then the log-likelihood ratio for the test for the null hypothesis $\theta_A = \theta_B$ 
Given two densities $\mu$ and $\nu$, and the flow parameter $\theta_T$, the maximum likelihood estimate of $\theta_A$ and $\theta_{BT}$ in (\ref{eq:m_def}) is given by
\begin{gather*}
   \langle \theta_A(\mu, \nu, \theta_T), \ \theta_{BT}(\mu, \nu, \theta_T) \rangle = \\ 
   = \argmax_{\theta_A, \theta_{BT}} \ME_{ab} g_F(a, b; \theta_T, \theta_A, \theta_{BT}) \ , \ a \sim \mu, \ b \sim \nu 
\end{gather*}
\end{definition}

\begin{definition}
Let us define the log-likelihood ratio distance $d_{\Lambda}(\mu, \nu, \theta_T)$ between $\mu$ and the pushforward measure $T(\nu, \theta)$ as the expected value of the test statistic for the log-likelihood ratio test for the null hypothesis:
$$ H_0: \theta_A(\mu, \nu, \theta_T) = \theta_{BT}(\mu, \nu, \theta_T) \triangleq \theta_{AT}. $$
It is equal to
\begin{gather*}
\begin{aligned}
\begin{split}
    d_{\Lambda}(\mu, \nu, \theta_T)
    = \max_{\theta_A, \theta_{BT}} \ME_{ab} & \ g_F(a, b; \theta_T, \theta_A, \theta_{BT}) \\
    - \max_{\theta_{AT}} \ME_{ab} & \ g_F(a, b; \theta_T, \theta_{AT}, \theta_{AT}) \\
    = \max_{\theta_A, \theta_{BT}} \min_{\theta_{AT}} \ME_{ab} \big[ & g_F(a, b; \theta_T, \theta_A, \theta_{BT})  \\ & - g_F(a, b; \theta_T, \theta_{AT}, \theta_{AT}) \big]
\end{split}
\end{aligned}
\end{gather*}
\end{definition}

\begin{lemma}
The log-likelihood ratio distance is always non-negative
$$ d_\Lambda(\mu, \nu, \theta_{T}) \geq 0$$
\end{lemma}
\begin{proof}
The second term in the definition of $d_\Lambda$ contains the same objective maximized over the smaller subset:
\begin{gather*} 
\max_{\theta_A, \theta_{BT}} \ME_{ab} g_F(a, b; \theta_T, \theta_A, \theta_{BT}) \\ \geq \max_{\theta_{AT}} \ME_{ab} g_F(a, b; \theta_T, \theta_{AT}, \theta_{AT}). 
\end{gather*}
\end{proof}

\begin{lemma}
If $\mu, \nu$ and $T(\nu)$ are from $\mathcal F$, i.e. 
\begin{gather*}
    \max_{\theta} \ME_{x \sim f} l_F(x; \theta) = \ME_{x \sim f} \log f(x), \ \forall f \in \{\mu, \nu, T(\nu)\}
\end{gather*} 
then
\begin{gather*}
    \max_{\theta_{BT}} \ME_{b} l_F(T(b; \theta_{T}); \theta_{BT}) \\ = \ME_{b} l_T(T(b; \theta_{T}); \theta_{T}) - \ME_{b} l_Z(b) + \max_{\theta_B} \ME_{b} l_F(b; \theta_B)
\end{gather*}

% $$ d_{\Lambda}(\mu, \nu, \theta_T) = \min_{\theta_{AT}}  \ME_{\mu\nu} l_T(T(b; \theta_T); \theta_T) - l_F(a; \theta_{AT}) - l_F(T(b; \theta_T); \theta_{AT}) + c(\mu, \nu) $$
% where the constant $c(\mu, \nu)$ does not depend on $\theta_{AT}$ and $\theta_T$ and can be precomputed, and the minimum of this value over $\theta_T$ is attained when $T$ transports $\nu$ to $\mu$, i.e. 
% $$ d(\mu, \nu, \theta_T) = 0 \iff \mu = T(\cdot, \theta_{T}) \# \nu $$
\end{lemma}

\begin{theorem}
For probability densities $\mu$, $\nu$ and the parametric normalizing flow $T(x; \theta)$ with log-likelihood $l_T(x; \theta)$, such that $\mu$, $\nu$ and $T(\nu)$ are from the same parametric family $\mathcal F$ with known log-likelihood $l_F(x; \theta)$, if there exist a flow parameter $\theta_T^*$ that minimizes the following objective and attains zero
\begin{gather}
    \min_{\theta_T} d'_\Lambda(\mu, \nu, \theta_{T}) = 0 \text{ , where }\\ 
    \begin{aligned}
    d'_\Lambda(\mu, \nu, \theta_{T}) = \min_{\theta_{AT}} \ME_{ab} \Big[ & l_T(T(b; \theta_T); \theta_T) - l_F(a; \theta_{AT}) \\ & - l_F(T(b; \theta_T); \theta_{AT}) + c(\mu, \nu) \Big]
\end{aligned}
\end{gather}
then it is equal to the log-likelihood ratio distance:
\begin{align*}
    d_\Lambda(\mu, \nu, \theta_{T}) = d'_\Lambda(\mu, \nu, \theta_{T})
\end{align*}
The constant
$$ c(\mu, \nu) = \max_{\theta_B} \ME_{b} l_F(b; \theta_B) + \max_{\theta_A} \ME_{a} l_F(a; \theta_A) - \ME_{b} l_Z(b) $$
does not depend on $\theta_{T}, \theta_{AT}$ and can be pre-computed in advance.
\end{theorem}

\begin{corollary}
The $\theta_T$ that minimizes the log-likelihood ratio distance can be found using iterative minimization (i.e. no adversarial min-max training), and the target function value at minimum has to equal zero. 
\end{corollary}

\begin{theorem}
The $\theta_T^*$ that minimizes the objective above also minimizes the adversarial integral probability measure
$$\min_{\theta_T} \max_{f \in \mathcal H} \Big[ \ME_{a} f(a) - \ME_{b} f(T(b; \theta_T)) \Big]$$
where
$$ \mathcal H = \{?\}$$
\end{theorem}

% \begin{example} Let us consider two unit variance distributions on the real line with means equal to zero and one respectively:
% \begin{gather*}
% a \sim \operatorname{Laplacian}\Big(0, \frac{1}{\sqrt{2}}\Big), \ \ 
% b \sim \operatorname{Exp}(1)
% \end{gather*}
% In this example we will restrict $\mathcal F$ to a Guassian family and $T(x; s, c) = c*x + s$ to affine transforms. 
% \end{example}

% The moments of original distributions are
% \begin{gather*}
%     \mu_a = 0, \mu_b = 1, 
%     \sigma_a^2 = 1, \sigma_b^2 = 1
% \end{gather*}
% The mean and the variance of the transformed $b$, and the variance of the mixture of the transformed $b$ with $a$ are:
% \begin{gather*}
%     \mu_{tb} = \mathbb{E} [ T(b; s, c) ] = s + 1 \\
%     \sigma_{tb}^2 = \mathrm{Var} [ T(b; s, c) ] = c^2 \sigma_b^2 = c^2 \\
%     \sigma_{at}^2 = \frac{1}{2} \Big(\sigma_a^2 + \sigma_{tb}^2 + \frac{1}{2}(\mu_a^2 + \mu_{tb}^2) - \mu_a \mu_{tb} \Big) \\
%     = \frac{1}{2} + \frac{1}{2} c^2 + 
% \end{gather*}

\begin{example}
Let us consider two random variables $A, B$ with moments $\mu_A, \mu_B, \sigma^2_A, \sigma^2_B$, restrict $\mathcal F$ to the Guassian family, and the transform $T(x; \theta)$ to the affine family: $T(x; a, b) = a*x + b$. The log-likelihood of the normal distribution depends on the variance as follows:
\begin{gather*}
    \max_{\mu, \sigma} \mathbb E_{X} l_F(X; \mu, \sigma) = -\frac{1}{2}\log(2\pi e \sigma_X^2) = C - \log \sigma_X
\end{gather*}
and the variance of the equal mixture can be expressed using moments of the mixture components $X$ and $Y$ as follows:
\begin{gather*}
    \sigma_{XY}^2 = \frac{1}{2}(\sigma^2_X + \sigma^2_Y) - \frac{1}{4}(\mu_X - \mu_Y)^2.
\end{gather*}
In our case
\begin{gather*}
    c(A, B) = 2C - \log \sigma_A - \log \sigma_B - \mathbb E \ l_Z(B) \\
    l_T(X; a, b) = - \log a + \mathbb E \ l_Z\Big[\frac{X-b}{a}\Big] \\
    l_T(T(B; a, b); a, b) = - \log a + \mathbb E \ l_Z(B)
\end{gather*}
we notice that the inner optimization problem can be solved analytically, which gives us the final expression for the log-likelihood ratio distance with Gaussian $\mathcal F$ and affine $T$ using the formula (3):
\begin{gather*}
    \min_{\mu_{AT}, \sigma_{AT}} \Big[ - l_F(A; \mu_{AT}, \sigma_{AT}) - l_F(T(B; \theta_T); \mu_{AT}, \sigma_{AT}) \Big] \\ 
    = -2C + \log\Big(\frac{1}{2}(\sigma_A^2 + a^2 \sigma_B^2) - \frac{1}{4}(\mu_A - \mu_B - b)^2 \Big) \\
    d_\Lambda(A, B, a, b) = - \log \sigma_A - \log \sigma_B - \log a \ + \\ + \log\Big(\frac{1}{2}(\sigma_A^2 + a^2 \sigma_B^2) - \frac{1}{4}(\mu_A - \mu_B - b)^2 \Big)
\end{gather*}
which can be solved analytically by setting the derivatives of wrt a and b to zero and gives us an intuitively meaningful parameters for the transformation that minimizes :
\begin{gather*}
a^* = \frac{\sigma_{A}}{\sigma_B}, \ \ \ b^* = \mu_A - \mu_B
\end{gather*}
\end{example}
\subsection{Alternative formulations}


==> old/3_method_old.tex <==
\section{Method}

In this section we introduce the log-likelihood ratio distance, and show that a normalizing flow that minimizes this distance can be found using a standard (non-adversarial) optimization. 

\subsection{Setup}
Consider a pair of distributions $P_A$ and $P_B$ over the shared domain $\mathcal X$, samples from respective distributions $A$ and $B$ of sizes $n$ and $m$. Our goal is to find a transformation $T(x)$ such that $T(B)$ is in some sense indistinguishable from $A$. We will consider a parametric family of log-likelihoods $l(x; \theta)$ and generator functions $G(x; \theta)$. 

\begin{definition}
We will call a triplet of functions $(l; G; P_z)$ \textbf{a conjugate generator triplet} on domain $\mathcal X$, latent space  $\mathcal Z$ isomorphic to $\mathcal X$, and the parameter space $\Theta$ if
\begin{enumerate}
    \item $l(x; \theta)$ is a log-likelihood function, i.e. $$\int_{\mathcal X} \exp\left(l(x; \theta)\right) dx = 1 \quad \forall \theta \in \Theta$$
    \item $G(z; \theta)$ is a smooth bijective mapping from the latent space to the domain $\mathcal X$ parameterized by $\theta \in \Theta$
    \item $P_z(z)$ is a prior distribution over the latent space
    \item The maximum of the log-likelihood function $l(x; \theta)$ evaluated on the dataset $G(z; \theta_0)$ for any parameter vector $\theta_0$ and a latent vector sampled from the prior $z \sim P_z(x)$ is attained at $\theta_0$ \begin{gather*}
    \max_{\theta \in \Theta} f(\theta_0, \theta) = f(\theta_0, \theta_0) \quad \forall \theta_0 \in \Theta \\ \text{ where } f(\theta_0, \theta_1) = \mathbb E_{z \sim P_z(z)} l\left(G(z; \theta_0); \theta_1\right) 
    \end{gather*}
\end{enumerate}
\end{definition}

\begin{notation}
We will denote the average log-likelihood over a dataset $X$ as 
$$  l(X; \theta) = \frac{1}{|X|} \sum_{x \in X} l(x; \theta)$$
\end{notation}    

\begin{definition} Consider two distributions $P_A$ and $P_B$, a log-likelihood function $l(x; \theta)$ parameterized by $\theta \in \Theta$, and a parametric model for a pair of samples from these distributions:
$$P(A, B \ | \ \theta_A, \theta_B) = \prod_{x \in A} \exp \big( l(x; \theta_A)\big) \cdot \prod_{x \in B} \exp\big( l(x; \theta_B) \big).$$ 

We will call a \textbf{log-likelihood ratio distance} $d_{\Lambda}(P_A, P_B)$ the value of the logarithm of the \textbf{likelihood ratio statistic} for a null hypothesis $\theta_A = \theta_B \triangleq \theta_{AB} $
\begin{align*}
d_{\Lambda}(P_A, P_B) = & - \log\left(\frac{\max_{\theta_{AB}} P(A, B \ | \ \theta_{AB}, \theta_{AB})}{\max_{\theta_{A}, \theta_{B}} P(A, B \ | \ \theta_A, \theta_B)}\right) \\
= & \max_{\theta_{A}} \mathbb E_{P_A} \ l(x; \theta_{A}) + \max_{\theta_{B}} \mathbb E_{P_A} \ l(x; \theta_{B}) \\
- & \max_{\theta_{AB}} \left[ \mathbb E_{P_A} \ l(x; \theta_{AB}) + \mathbb E_{P_B} \ l(x; \theta_{AB}) \right].
% \text{ where } L&(P, \theta) = \mathbb E_{x \sim P} \ l(x; \theta) 
\end{align*}
It has an empirical estimator
\begin{align*}
d_{\Lambda}(A, B) = 
& \max_{\theta_{A}} \  l(A; \theta_{A}) + \max_{\theta_{B}} \  l(B; \theta_{B}) \\
- & \max_{\theta_{AB}} \left[  l(A; \theta_{AB} ) +  l(B; \theta_{AB}) \right].
\end{align*}
\end{definition}

\begin{theorem}
Given a conjugate generator triplet $(l; G; P_z)$ and samples from two distributions $A \sim P_A, B \sim P_B$ the log-likelihood ratio distance between a fixed set of samples $A$ and a set of transformed samples $T \triangleq G(B; \theta_T)$ is equal to
\begin{gather*}
d_{\Lambda}\left(A, T\right) = \min_{\theta_{AB}} \big( l(T; \theta_{T}) -  l(A; \theta_{AB} ) -  l(T; \theta_{AB}) + c \big)
\end{gather*}
Where the constant 
$$ c =  \max_{\theta} \ l(A; \theta) + \max_{\theta} \ l(B; \theta) - \log P_z(B) $$
depends only on original datasets $A$ and $B$, does not depend on $\theta_{AB}$ and $\theta_T$, and can be pre-computed before the optimization takes place advance.
\end{theorem}

\begin{proof}
To prove it by contradiction try and assume that the statemenet is false,
proceed from there and at some point you will arrive to a contradiction.
\end{proof}

\begin{corollary}
The minimum of the log-likelihood ratio distance can be found by 
\end{corollary}

If used plain KL-divergence, the result would be ill-defined for distributions with non-overlapping supports.

==> old/lemma.tex <==

\begin{lemma}
If $M$ can approximate $A \sim P_A$ well, i.e.
$$\min_{\theta} L(A; \theta) = - \log P_A(A)$$
where $P_A$ is the true data distribution of $A$, and if $T(x; \phi)$ is the family of normalizing flows from $\mathcal X$ to itself, then the amount of additional entropy (negative log-likelihood) the transformation $T(x, \phi)$ induces upon $A$ according to $M$ is bounded by the actual amount of entropy it induces upon it: 
% the probability density function $P_T(x, \phi)$ and the prior density $P_Z(x)$, then
\begin{equation*}
\begin{gathered}
    \min_{\theta_{AT}} L(T(A, \phi); \theta_{AT}) - \min_{\theta_{A}} L(A; \theta_{A})\\ 
    %     \geq \log P_Z(A) - \log P_T(T(A, \phi), \phi) + \min_{\theta_{A}} L(A; \theta_{A}).
    \geq - \log \det | \nabla_x T_{\phi}^{-1}(T_\phi(A))|.
\end{gathered}
\end{equation*}
\end{lemma}
\begin{proof}
We know from the change of variable formula that if $T_{\phi}$ is a normalizing flow and $X = T_{\phi}(Z)$ where $Z \sim P_Z$, then the log-likelihood can be expressed as
$$\log P^Z_T(X|\phi) = \log P_Z(T_{\phi}^{-1}(X)) + \log \det | \nabla_x T_{\phi}^{-1}(X) |.$$ 

Following the same logic, if $A' = T_{\phi}(A)$ and $A \sim P_A$, and considering the invertibility of $T_{\phi}$, we can express the true distribution of $A'$ as follows (the superscript in $P_T^A$ indicates that we used $P_A$ instead of $P_Z$ in that flow likelihood):
\begin{align*}
    \log P^A_T(A'|\phi) & = \log P_A(T_{\phi}^{-1}(T_{\phi}(A)) + \log \det | \nabla_x T_{\phi}^{-1}(T_{\phi}(A)) | \\
    & = \log P_A(A) + \log \det | \nabla_x T_{\phi}^{-1}(T_{\phi}(A)) |
    % & = \log P_A(A) + \log P^Z_T(T_{\phi}(A)|\phi) - \log P_Z(T_{\phi}^{-1}(T_{\phi}(A)) \\
    % & = \log P_A(A) + \log P^Z_T(T_{\phi}(A)|\phi) - \log P_Z(A).
\end{align*}
% The second line expresses the log-determinant term using the definition of $\log P_T^Z$ provided above. 
Considering that $M$ can approximate $A$ well, i.e. $- \min_{\theta} L(A; \theta) = \log P_A(A)$, but might not approximate the true distribution of the transformed dataset $P_T^A$ as well:
\begin{gather*}
    - \min_{\theta} L(A'; \theta) \leq \log P^A_T(A'|\phi) \ \Rightarrow\\
    - \min_{\theta} L(A'; \theta) \leq - \min_{\theta} L(A; \theta) + \log \det | \nabla_x T_{\phi}^{-1}(T_{\phi}(A)) |
\end{gather*}
after multiplying both sides by negative one and reordering the terms we get the statement of the lemma.
\end{proof}
